A General Framework for Evaluating Callout Mechanisms in Repeated Auctions

Motivated by online display ad exchanges, we study a setting in which an exchange repeatedly interacts with bidders who have quota, making decisions about which subsets of bidders are called to participate in ad-slot-specific auctions. A bidder with quota cannot respond to more than a certain number of calls per second. In practice, random throttling is the principal solution by which these constraints are enforced. Given the repeated nature of the interaction with its bidders, the exchange has access to data containing information about each bidder's segments of interest. This information can be utilized to design smarter callout mechanisms --- with the potential of improving the exchange's long-term revenue. In this work, we present a general framework for evaluating and comparing the performance of various callout mechanisms using historical auction data only. To measure the impact of a callout mechanism on long-term revenue, we propose a strategic model that captures the repeated interaction between the exchange and bidders. Our model leads us to two metrics for performance: immediate revenue impact and social welfare. Next we present an empirical framework for estimating these two metrics from historical data. For the baseline to compare against, we consider random throttling, as well as a greedy algorithm with certain theoretical guarantees. We propose several natural callout mechanisms and investigate them through our framework on both synthetic and real auction data. We characterize the conditions under which each heuristic performs well and show that, in addition to being computationally faster, in practice our heuristics consistently and significantly outperform the baselines.

==> figures.tex <==
\section{Omitted Figures and Plots}\label{app:figs}

\begin{figure}[h!]
\centering 
\includegraphics[width=0.6\textwidth]{flowchart.pdf}
\caption{The high-level flowchart of the system. The two main building blocks of a callout mechanism are the components for \textit{learning} and \textit{targeting}. We treat the auction mechanism as fixed and given throughout.} \label{fig:flowchart}
\end{figure}

\begin{figure}[h!] 
\centering 
\includegraphics[width=0.7\textwidth]{baseline.png}
\caption{A good callout mechanism (red) must exceed the baselines RQT (blue) and GRA (cyan) in terms of revenue (left panel) while maintaining social welfare at least as large as RQT (right panel).} 
\label{fig:baseline}
\end{figure}


\begin{figure*}[t!]
       \centering
\subfigure{\includegraphics[width=0.32\textwidth]{figures/rv-n100m100r10mu1v1.png}}
\subfigure{\includegraphics[width=0.32\textwidth]{figures/rv-n100m100r10mu1v5.png}}
\subfigure{\includegraphics[width=0.32\textwidth]{figures/rv-n100m100r10mu1v10.png}}
\subfigure{\includegraphics[width=0.32\textwidth]{figures/sw-n100m100r10mu1v1.png}}
\subfigure{\includegraphics[width=0.32\textwidth]{figures/sw-n100m100r10mu1v5.png}}
\subfigure{\includegraphics[width=0.32\textwidth]{figures/sw-n100m100r10mu1v10.png}}
\subfigure{\includegraphics[width=0.32\textwidth]{figures/scores-n100m100r10mu1v1.png}}
\subfigure{\includegraphics[width=0.32\textwidth]{figures/scores-n100m100r10mu1v5.png}}
\subfigure{\includegraphics[width=0.32\textwidth]{figures/scores-n100m100r10mu1v10.png}}

        \caption{The effect of variance on the performance of each callout mechanism. Here $T=100$ and $r=1$.}
         \label{fig:variance}
\end{figure*}

\begin{figure*}[t!]
       \centering
\subfigure{\includegraphics[width=0.32\textwidth]{figures/rv-n100m50r10mu1v10.png}}
\subfigure{\includegraphics[width=0.32\textwidth]{figures/rv-n100m100r10mu1v10.png}}
\subfigure{\includegraphics[width=0.32\textwidth]{figures/rv-n100m200r10mu1v10.png}}
\subfigure{\includegraphics[width=0.32\textwidth]{figures/sw-n100m50r10mu1v10.png}}
\subfigure{\includegraphics[width=0.32\textwidth]{figures/sw-n100m100r10mu1v10.png}}
\subfigure{\includegraphics[width=0.32\textwidth]{figures/sw-n100m200r10mu1v10.png}}
\subfigure{\includegraphics[width=0.32\textwidth]{figures/scores-n100m50r10mu1v10.png}}
\subfigure{\includegraphics[width=0.32\textwidth]{figures/scores-n100m100r10mu1v10.png}}
\subfigure{\includegraphics[width=0.32\textwidth]{figures/scores-n100m200r10mu1v10.png}}

        \caption{The effect of $T$ on the performance of each callout mechanism. Here $r=1$ and $\sigma= 1$.}
         \label{fig:m}
\end{figure*}



